Conformal Modules

In this paper we study a class of modules over infinite-dimensional Lie (super)algebras, which we call conformal modules. In particular we classify and construct explicitly all irreducible conformal modules over the Virasoro and the N=1 Neveu-Schwarz algebras, and over the current algebras.

==> erratum.tex <==
\magnification=\magstep1
\baselineskip=18pt
\font\bbd = msbm10 at 10pt
\font\bbds = msbm8 at 8pt
\font\bbds = msbm7 at 8pt
\font\csc = cmcsc10 at 10pt
\font\small = cmr8 at 8pt
\font\frak = eufm10 at 10pt
\font\fraksmall = eufm8 at 8pt
\font\xmplbx = cmbx10 scaled \magstep1
\outer\def\beginsection#1{\vskip 0pt plus.3\vsize\penalty-10
                          \vskip 0pt plus-.3\vsize\bigskip\medskip\vskip\parskip
                          \message{#1}\leftline{\bf #1}
                          \nobreak\smallskip}
\outer\def\proclaim #1 #2\par{\medbreak
      \noindent{\bf#1\enspace}{\sl#2}\par
      \ifdim\lastskip<\medskipamount \removelastskip\penalty55\medskip\fi}
\def\proof {\noindent {\it Proof.} \ \ }
\def\remark {\noindent {\it Remark.} \ \ }
\def\remarks {\noindent {\it Remarks.} \ \ }
\def\definition {\noindent {\bf Definition.} \ \ }
\def\sqr#1#2{{\vcenter{\hrule height.#2pt
              \hbox{\vrule width.#2pt height#1pt \kern#1pt \vrule width.#2pt}
                    \hrule height.#2pt}}}
\def\qe{\mathchoice\sqr54\sqr54\sqr{2.1}3\sqr{1.5}3}
\def\blackbox{\vrule height6pt depth-1pt width5pt}
\def\qed{\quad\qe}
\def\square{\hbox{$\sqr54$}}
\def\mapright#1{\smash{\mathop{\longrightarrow}\limits^{\scriptstyle#1}}}
\def\chainmap#1{\smash{\mathop{\rightarrow}\limits^{\scriptstyle#1}}}
\def\mapdown#1{\Big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\smapdown#1{\big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\C{\mathord{\hbox{\bbd C}}}
\def\c{\mathord{\hbox{\bbds C}}}
\def\Cl{\mathord{\hbox{\scriptstyle C}}}
\def\F{\mathord{\hbox{\bbd F}}}
\def\N{\mathord{\hbox{\bbd N}}}
\def\form{(\cdot|\cdot)}
\def\Q{\mathord{\hbox{\bbd Q}}}
\def\D{\mathord{\hbox{\frak D}}}
\def\V{\mathord{\hbox{\frak V}}}
\def\v{\mathord{\hbox{\fraksmall V}}}
\def\d{\mathord{\hbox{\fraksmall D}}}
\def\a{\mathord{\hbox{\fraksmall a}}}
\def\A{\mathord{\hbox{\frak a}}}
\def\b{\mathord{\hbox{\fraksmall b}}}
\def\B{\mathord{\hbox{\frak b}}}
\def\F{\mathord{\hbox{\frak F}}}
\def\g{\mathord{\hbox{\fraksmall g}}}
\def\G{\mathord{\hbox{\frak g}}}
\def\n{\mathord{\hbox{\frak n}}}
\def\NS{\mathord{\hbox{\frak N}}}
\def\ns{\mathord{\hbox{\fraksmall N}}}
\def\l{\mathord{\hbox{\fraksmall L}}}
\def\L{\mathord{\hbox{\frak L}}}
\def\h{\mathord{\hbox{\fraksmall h}}}
\def\H{\mathord{\hbox{\frak h}}}
\def\u{\mathord{\hbox{\frak U}}}
\def\s{\mathord{\hbox{\frak s}}}
\def\Re{\mathord{\hbox{\bbd R}}}
\def\Z{\mathord{\hbox{\bbd Z}}}
\def\k{\mathord{\hbox{\frak k}}}
\def\z{\mathord{\hbox{\bbds Z}}}
\def\lsemi{\mathbin{\hbox{\bbd n}}}
\def\lsemis{\mathbin{\hbox{\bbds n}}}
\def\rsemi{\mathbin{\hbox{\bbd o}}}
\def\rsemis{\mathbin{\hbox{\bbds o}}}
\def\ind{\mathord{\hbox{Ind}}}
\def\subsetneq{\mathbin{\hbox{\bbd (}}}
\def\inv#1{#1^{-1}}
\def\setbrackets #1 #2{\bigr\{\,#1\bigm|#2\,\bigr\}}
\def\w#1{\widehat{#1}}
\def\dd{\mathord{\hbox{$\partial$}}}
\def\dt{\mathord{\hbox{${d\over{d t}}$}}}

\centerline { \xmplbx Erratum: Conformal Modules}
\medskip
\centerline { by }
\medskip
\centerline {Shun-Jen Cheng{$^\dagger$}
 and Victor G. Kac{$^{\dagger\dagger}$}}
\medskip
\vbox{\small\baselineskip=10pt  $^\dagger$Department of Mathematics,
National Cheng-Kung University, Tainan,
Taiwan\hfill\break\indent\phantom{$^\dagger$}chengsj@mail.ncku.edu.tw}
\medskip
\vbox{\small\baselineskip=10pt $^{\dagger\dagger}$Department of Mathematics,  
MIT, Cambridge, MA 02139,
USA\hfill\break\indent\phantom{$^\dagger\dagger$}kac@math.mit.edu}
\vskip 0.5in

In this erratum we make corrections (a),(b) and (c) to our paper [3].

(a) Here is a correct statement and a proof of Lemma 3.2 of [3].

\proclaim{Lemma 1.} Let $\G$ be a finite-dimensional Lie superalgebra
and let $\n$ be a solvable
ideal of $\G$.  Let $\A$ be an even subalgebra of
$\G$ such that $\n$ is a completely reducible ${\rm ad}\A$-module with no
trivial summand.
Then $\n$ acts trivially in any irreducible finite-dimensional
$\G$-module $V$.

\proof First note that if $[a,b]=b$, then $b$ is nilpotent on any
finite-dimenisonal representation $V$.  To see this, note that if $v\in V$ is  
an eigenvector of $a$ with eigenvalue $\lambda$, then the condition
$[a,b]=b$ implies that $bv$ is an eigenvector of $a$ with eigenvalue
$\lambda+1$.  Thus there exists a non-zero $w\in V$ such that $bw=0$.  Let
$W$ be the space annihilated by $b$.  Then $W$ is $a$-invariant.  Since
$W\not=0$, it follows by induction on the dimension of $V$ that $b$ is
nilpotent on $V/W$.  Thus $b$ is nilpotent on $V$.

Let $\s$ be an
irreducible ${\rm ad}\A$-submodule of $\n$. By the assumption, it is a
module with a non-zero highest weight.
Hence there
exists $a\in\A$ and $b\in\s$ such that $[a,b]=b$, therefore $b$
is nilpotent on $V$.  Moreover all elements from the orbit ${\rm Ad}A\cdot
b$, where $A$ is the connected Lie group with Lie algebra $\A$, are
nilpotent on $V$.  Since $\s$ is ${\rm Ad}A$-irreducible, this orbit
spans $\s$, hence $\s$ is spanned by elements that are
nilpotent on $V$.  Thus any $\A$-submodule of  $\n$ is spanned by elements
that are nilpotent on
$V$.

To prove the lemma, we may assume that $V$ is a faithful
$\G$-module.  Suppose
the lemma is not true, i.e.~$\n$ is non-zero.  Let $\n^{(i)}$ be the last
non-zero member of its derived series. By the above, $\n^{(i)}$ is spanned by
mutually commuting elements that are nilpotent on $V$, and hence $\n^{(i)}$  
annihilates a non-zero vector in $V$.
But $\n^{(i)}$ is an ideal of $\G$ and hence the subspace of $V$,
annihilated by $\n^{(i)}$, is a $\G$-submodule of $V$.  Thus $\n^{(i)}$
annihilates $V$ and so $V$ is not faithful, which is a contradiction. $\qed$

(b) Lemma 1, however, is not applicable to the current algebra of three series  
of simple Lie superalgebras that we have considered in [3].  Namely the Lie  
superalgebras $A(m|n)$, for $m\not=n$, $C(n)$ and $W(n)$ (see [4]) for which  
$\n$ will contain trivial summands.  For these three series the statement of  
Corollary 3.1 and Theorem 3.2 turns out to be incorrect.  Below we will classify irreducible  
conformal modules over their current algebras.  Due to Lemma 3.1 of [3]  
it suffices to consider finite-dimensional irreducible representations of the  
Lie superalgebra $\G\otimes\C[t]/t^{n+1}$, where $n\ge 0$ and $\G$ is a  
member of one of the three series of simple Lie superalgebras above.  As the  
case of $n=0$ is trivial, we may assume from now on that $n\ge 1$.  In fact  
we will study more general Lie superalgebras $\G$ satisfying properties we  
now describe.

Let $\G=\G_{\bar{0}}\oplus\G_{\bar{1}}$ be a finite-dimensional Lie  
superalgebra and suppose that  
$\G=\G_{-1}\oplus\G_{0}\oplus\G_{1}\oplus\G_{2}\oplus\cdots\oplus\G_{k}$ is  
$\Z$-graded such that $\G_{i}\subseteq\G_{\bar{i}}$. Assume that  
$\G_{0}=\A\oplus\C c$ is a reductive Lie algebra such that $\A$ is a  
semisimple subalgebra and $c$ is a central element.  Furthermore suppose that  
$\G_i$ as an $\A$-module has no trivial summand for $i\not=0$, and there  
exists an $\A$-submodule $\G_{-1}^*\subseteq\G_{1}$ contragredient to  
$\G_{-1}$ and $\G_{1}=\G_{-1}^*\oplus\G_1'$ as $\A$-modules with  
$[\G_{1}',\G_{-1}]\subseteq\A$.  Finally suppose that given any non-zero  
$a\in\G_{-1}$ $[a,\G_{-1}^*]\cap\C c\not=0$ and given any non-zero  
$b\in\G_{-1}^*$ $[\G_{-1},b]\cap\C c\not=0$.  Note that it follows from the  
descriptions of the three series of simple Lie superalgebras $A(m|n)$, for  
$m\not=n$, $C(n)$ and $W(n)$ in [4] that they satisfy the assumptions of $\G$  
above.

Set $\L=\G\otimes\C[t]/t^{n+1}$.  We want to determine finite-dimensional  
irreducible $\L$-modules, on which $\G\otimes t^n$ acts non-trivially.  We  
let
$$G_{0}=\G_{0}+\G_1'+\sum_{i\ge 2}\G_{i}.$$
Consider the subalgebra $L\subseteq\L$, which is defined as follows:
For $n=2k$, $k\in\N$, an even integer, we let
$$L:=G_{0}+G_{0}\otimes t+\cdots+G_{0}\otimes t^{k-1}+(G_{0}+\G_{1})\otimes  
t^{k}+\G\otimes t^{k+1}+\cdots+\G\otimes t^{2k}.$$
If $n=2k+1$ is odd, then we let
$$L:=G_{0}+G_{0}\otimes t+\cdots+G_{0}\otimes t^{k}+\G\otimes  
t^{k+1}+\cdots+\G\otimes t^{2k+1}.$$
We first determine finite-dimensional irreducible $L$-modules.  It will turn  
out that every irreducible $\L$-module on which $\G\otimes t^n$ acts  
non-trivially are obtained from inducing from a suitable irreducible  
$L$-module.  The main tool we use to prove this assertion is the Lie  
algebraic analogue of Mackey's irreducibility criterion [1].  Before  
recalling it, we need some terminology. Let $\k$ be a finite-dimensional Lie  
superalgebra and $I\subseteq\k$ be an ideal of $\k$.  Let $(\pi,V_{I})$ be an  
irreducible $I$-module.  Define the stabilizer associated to the pair  
$(\pi,I)$ to be $K_{\pi}=\{k\in\k|\exists A_k\in{\rm End}(V_{I}){\rm\ with\ }  
\pi([k,i])=[A_k,\pi(i)],\forall i\in I\}$. $K_{\pi}$ is a subalgebra  
containing $I$.  One can prove using analogous arguments as in [1]

\proclaim{Theorem 1. [2]} Let $V_{K}$ be an irreducible representation of  
$K_{\pi}$ such that as an $I$-module, $V_{K}$ is a direct sum of copies of  
$\pi$.  If the $\Z_2$-graded space $\k/K_{\pi}$ is spanned by elements of the  
same parity, then ${\rm Ind}_{K_{\pi}}^{\k}V_{K}$ is an irreducible  
$\k$-module.

We now consider the subalgebra
$$B=\B+\G_1'+\sum_{i\ge 2}\G_i+(L\cap\G\otimes\C[t]t),$$
where $\B$ is a Borel subalgebra of $\G_{0}$.  Then $B$ is a solvable  
subalgebra of $L$ and $[B_{\bar{1}},B_{\bar{1}}]\cap\C c=0$.  However, since  
$\G$ as an $\A$-module contains only one trivial summand, namely $\C c$, it  
is clear that $[\B,\G_i]=\G_i$, for all $i\not=0$, and $[\B,\G_0]=\A$.  In  
fact $[\B,\G_{-1}^*]=\G_{-1}^*$ and $[\B,\G_{1}']=\G_{1}'$.  This discussion  
implies  that $[B_{\bar{1}},B_{\bar{1}}]\subseteq [B_{\bar{0}},B_{\bar{0}}]$.  
 Therefore by [4] every finite-dimensional irreducible representation of $B$  
is one-dimensional, say $\C v_{\lambda}$, where $\lambda:\H+\C  
c\otimes\C[t]\rightarrow\C$ is a linear form extended trivially to $B$ and  
$\H$ is a Cartan subalgebra in $\B$.  However ${\rm Ind}_{B}^{L}\C  
v_{\lambda}$ is spanned by elements of the form  
$e_{-\alpha_1}^{k_{\alpha_1}}\cdots e_{-\alpha_m}^{k_{\alpha_m}}v_{\lambda}$,  
where $e_{-\alpha_j}$ are negative root vectors of $\A$.  It follows that  
$c\otimes t^j$ acts as a scalar on ${\rm Ind}_{B}^{L}\C v_{\lambda}$.  Set $\G^c=\G_{-1}+\A+\sum_{i\ge 1}\G_i$.  Clearly $[\A,\G^{c}]=\G^{c}$. From this it follows by induction on $k_{\alpha_1}+\cdots+k_{\alpha_m}$ that $\G_1'+\sum_{i\ge  
2}\G_i+(\G^c\otimes\C[t]t)\cap L$ acts trivially on  
this induced module. Thus we obtain

\proclaim{Proposition 1.} Every irreducible $L$-module is an irreducible  
$\G_0\oplus (c\otimes\C [t]t)$-module, on which $\G_1'+\sum_{i\ge  
2}\G_i+(\G^c\otimes\C[t]t)\cap L$ acts trivially.

Next we introduce the auxilary subalgebra
$$\bar{\L}:=G_{0}+\G\otimes\C[t]t.$$
From Proposition 1 we obtain the classification of finite-dimensional  
irreducible $\bar{\L}$-modules.

\proclaim{Proposition 2.}  Let $V_{L}$ be an irreducible $L$-module such  
that $c\otimes t^n$ acts as a non-zero scalar.  Then ${\rm  
Ind}_{L}^{\bar{\L}}V_{L}$ is irreducible.  Furthermore suppose that  $W$ is  
an irreducible $\bar{\L}$-module on which $\G\otimes t^n$ acts non-trivially,  
then $W\cong{\rm Ind}_{L}^{\bar{\L}}V_{L}$, where $V_{L}$ is as above.

\proof Let $I=(G_0+\G_1)\otimes t^k+\G\otimes\C[t]t^{k+1}$, if $n=2k$ and  
$I=\G\otimes\C[t]t^{k+1}$, if $n=2k+1$. Note that $I$ is an ideal of  
$\bar{\L}$. By Proposition 1 $V_{L}$ is a direct sum of $1$-dimensional  
mutually isomorphic $I$-modules $\C v_{\lambda}$, where $(c\otimes t^j)  
v_{\lambda}=\lambda(c\otimes t^j) v_{\lambda}$.  Consider the stabilizer of  
the $I$-module $\C v_{\lambda}$ in $\bar{\L}$.  Since for every vector  
$g\in\G_{-1}+\G_{-1}^*$ there exists a vector $g'\in\G_{-1}+\G_{-1}^*$ such  
that $[g,g']=\mu c+a$, where $\mu\not=0$ and $a\in\A+\G_2$, it follows that the  
stabilizer is precisely $L$, if $\lambda(c\otimes t^n)\not=0$.  Since also  
$\bar{\L}/L$ is a completely odd vector space, we can employ Theorem 1 and  
irreducibility follows.  On the other hand suppose that $W$ is an irreducible  
$\bar{\L}$-module on which $\G\otimes t^n$ acts non-trivially.  Let $V_{L}$  
be an irreducible $L$-submodule inside $W$.  If $c\otimes t^n$ acts trivially  
on $V_L$, then $\G\otimes t^n$ acts trivially on $V_L$ by Proposition 1.   
But  $\G\otimes t^n$ is an ideal of $\bar{\L}$ and hence acts trivially on  
$W$, which is a contradiction.  $\qed$

Proposition 1 says that inducing from $L$ to $\bar{\L}$ irreducibility is  
preserved.  So our final goal is to show that induction from $\bar{\L}$ to  
$\L$ also preserves irreducibility.  Note that from Proposition 2 we get

\proclaim{Corollary 1.} Every irreducible $\bar{\L}$-module, on which  
$\G\otimes t^n$ acts non-trivially, considered as a $\G\otimes t^n$-module,  
is a direct sum of the same $1$-dimensional $\G\otimes t^n$-module $\C  
v_{\lambda}$.  Furthermore $c\otimes t^n$ acts as a non-zero scalar $  
{\lambda}(c\otimes t^n)$, while $\G^c\otimes t^n$  
acts trivially.

Now we are ready to classify irreducible $\L$-modules.

\proclaim{Proposition 3.} Let $V$ be an irreducible $\bar{\L}$-module on  
which $c\otimes t^n$ acts as a non-zero scalar.  Then ${\rm  
Ind}_{\bar{\L}}^{\L}V$ is an irreducible $\L$-module.  Furthermore every  
irreducible $\L$-module, on which $\G\otimes t^n$ acts non-trivially, is of  
this form.

\proof  We will set up to employ Theorem 1 again.  By Corollary 1 $V$ is a  
direct sum of copies of the $\G\otimes t^n$-module $\C v_{\lambda}$ and  
$\lambda(c\otimes t^n)\not=0$.  We compute the stabilizer of the $\G\otimes  
t^n$-module $\C v_{\lambda}$ now in $\L$.  Again using the same argument as  
in the proof of Proposition 2, one checks that the stabilizer is precisely  
$\bar{\L}$, if $\lambda(c\otimes t^n)\not=0$.  Thus by Blattner's theorem  
again, the induced module is irreducible.  The same argument as in  
Proposition 2 gives that these are all such irreducibles.  $\qed$

Combining Proposition 2 and 3 gives

\proclaim{Theorem 2.} All finite-dimensional irreducible representations of  
$\L$, on which $\G\otimes t^n$ acts non-trivially, are of the form ${\rm  
Ind}_{L}^{\L}V_{L}$, where $V_{L}$ is an irreducible representation of $L$,  
on which $c\otimes t^n$ acts as a non-zero scalar.  Furthermore all such  
representations are irreducible.

In [2] it was shown that if $S$ is a finite-dimensional Lie superalgebra  
such that $[S,S]=S$ and $\Lambda(n)$ is the Grassmann superalgebra in $n$ odd  
variables, then every finite-dimensional irreducible  
$S\otimes\Lambda(n)$-module is an irreducible $S$-module, on which the  
$S\otimes N$ acts trivially, where $N$ is the maximal nilpotent ideal of  
$\Lambda(n)$.  Thus for supercurrents  
$\G[t,\theta]=\G\otimes\C[t,t^{-1}]\otimes\Lambda(1)$, where $\theta$ is an  
odd variables and $\G$ is one of the three series of simple Lie  
superalgebras, we may apply this result and Theorem 2 to obtain their  
irreducible conformal modules.

(c) In the proof of Lemma 3.1 in [3] we use $v$
to denote the vector $\sum_{i=1}^n{p_i(\dd)v_i}$.



\bigskip
\centerline  {\bf REFERENCES }
\bigskip
\frenchspacing
\medskip

\item{1.} Blattner, R.J.: Induced and Produced Modules of Lie Algebras,  
Trans.~AMS, {\bf 144} (1969) 457--474.

\item{2.} Cheng, S.-J.: Differentiably Simple Lie Superalgebras and  
Representations of Semisimple Lie superalgebras, J.~Alg., {\bf 173} (1995)  
1--43.

\item{3.} Cheng, S.-J.; Kac, V.G.: Conformal Modules, Asian J.~Math., {\bf
Vol.}~1, No.~1 (1997) 181--193.

\item{4.} Kac, V.G.: Lie Superalgebras, Adv.~in Math.,~{\bf 26} (1977) 8--96.

\end











